SVDistNet: Self-Supervised Near-Field Distance Estimation on Surround View Fisheye Cameras

A 360{\deg} perception of scene geometry is essential for automated driving, notably for parking and urban driving scenarios. Typically, it is achieved using surround-view fisheye cameras, focusing on the near-field area around the vehicle. The majority of current depth estimation approaches focus on employing just a single camera, which cannot be straightforwardly generalized to multiple cameras. The depth estimation model must be tested on a variety of cameras equipped to millions of cars with varying camera geometries. Even within a single car, intrinsics vary due to manufacturing tolerances. Deep learning models are sensitive to these changes, and it is practically infeasible to train and test on each camera variant. As a result, we present novel camera-geometry adaptive multi-scale convolutions which utilize the camera parameters as a conditional input, enabling the model to generalize to previously unseen fisheye cameras. Additionally, we improve the distance estimation by pairwise and patchwise vector-based self-attention encoder networks. We evaluate our approach on the Fisheye WoodScape surround-view dataset, significantly improving over previous approaches. We also show a generalization of our approach across different camera viewing angles and perform extensive experiments to support our contributions. To enable comparison with other approaches, we evaluate the front camera data on the KITTI dataset (pinhole camera images) and achieve state-of-the-art performance among self-supervised monocular methods. An overview video with qualitative results is provided at https://youtu.be/bmX0UcU9wtA. Baseline code and dataset will be made public.

==> img/cam_tensor/cam_tensor_qual.tex <==
\begin{comment}
\newcommand{\imlabel}[2]{\includegraphics[width=.49\textwidth]{#1}
\raisebox{2pt}{\makebox[-2pt][r]{\small #2}}}

\scalebox{1}[1]{
\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0mm}c@{\hskip 0mm}c}
\centering
    \imlabel{img/cam_convs/20190614_164033_1127_crop.jpg}
    {\textcolor{white}{Front Cam}} &
    \imlabel{img/cam_convs/20190614_161909_429.jpg}
    {\hspace{.1\textwidth}\textcolor{white}{Right Cam}}  \\

    \imlabel{img/cam_convs/20190614_164033_1127_fish_cam_conv.png}
    {\hspace{.1\textwidth}\textcolor{purple}{Fisheye-Cam-Conv}} &
    \imlabel{img/cam_convs/20190614_161909_429_fish_cam_conv.png}
    {\hspace{.1\textwidth}\textcolor{purple}{Fisheye-Cam-Conv}} \\
    
    \imlabel{img/cam_convs/20190614_164033_1127_no_fish_cam_conv.png}
    {\hspace{.35\textwidth}\textcolor{purple}{No Fisheye-CamConv}}  &
    \imlabel{img/cam_convs/20190614_161909_429_fish_no_cam_conv.png}
    {\hspace{.35\textwidth}\textcolor{purple}{No Fisheye-CamConv}}  \\

\end{tabular}
}
\end{comment}

\newcommand{\turnheightnew}{0.5\columnwidth}
\centering
\large
\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

{\rotatebox{90}{\hspace{1mm}}} &
\includegraphics[height=\turnheightnew]{img/cam_tensor/20190614_164033_1127_crop.jpg} &
\includegraphics[height=\turnheightnew]{img/cam_tensor/20190614_161909_429.jpg}\\

{\rotatebox{90}{\hspace{1mm}}} &
\includegraphics[height=\turnheightnew]{img/cam_tensor/20190614_164033_1127_fish_cam_conv.png} &
\includegraphics[height=\turnheightnew]{img/cam_tensor/20190614_161909_429_fish_cam_conv.png}\\

{\rotatebox{90}{\hspace{1mm}}} &
\includegraphics[height=\turnheightnew]{img/cam_tensor/20190614_164033_1127_no_fish_cam_conv.png} &
\includegraphics[height=\turnheightnew]{img/cam_tensor/20190614_161909_429_fish_no_cam_conv.png} \\

\end{tabular}

\begin{comment}
\newcommand{\turnheightnew}{0.5\columnwidth}
\centering
\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_164033_1127_crop.jpg} &
\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_164033_1127_fish_cam_conv.png} &
\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_164033_1127_no_fish_cam_conv.png} \\

\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_161909_429.jpg} &
\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_161909_429_fish_cam_conv.png} &
\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_161909_429_fish_no_cam_conv.png} \\

\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_161909_292_crop.jpg} &
\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_161909_292_fish_cam_conv.png} &
\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_161909_292_no_fish_cam_conv.png} \\


\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_164033_973_crop.jpg} &
\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_164033_973_fish_cam_conv.png} &
\includegraphics[height=\turnheightnew]{img/cam_convs/20190614_164033_973_no_fish_cam_conv.png} \\
\end{tabular}
\end{comment}


==> img/failure_case/failure_case.tex <==
\newcommand{\turnheightnew}{0.25\columnwidth}
\centering

\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

{\rotatebox{90}{\hspace{0mm}}} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000555_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000879_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000294_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000603_cropped.jpg}\\

{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000555_box.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000879_box.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000294_box.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000603_box.jpg} \\

\end{tabular}


==> img/fisheye_fig/fisheye_qualitative.tex <==
\newcommand{\turnheightnew}{0.25\columnwidth}
\centering
\setlength{\extrarowheight}{-0.5pt}
\begin{tabular}{@{\hskip 0.4mm}c@{\hskip 0.4mm}c@{\hskip 0.4mm}c@{\hskip 0.4mm}c@{\hskip 0.4mm}c@{\hskip 0.4mm}}

{\rotatebox{90}{\hspace{0mm}}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_143708_448_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_143708_528_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164033_Scene1_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164537_14_cropped.jpg}\\

{\rotatebox{90}{\hspace{0mm}}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_143708_448_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_143708_528_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164033_Scene1_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164537_14_norm.jpg}\\

% Distortion
{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164033_Scene2_1138_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_537_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_161909_405_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164033_Scene2_1083_cropped.jpg} \\

{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164033_Scene2_1138_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_537_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_161909_405_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164033_Scene2_1083_norm.jpg} \\

% Sharp Edges
{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_340_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_368_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_152_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_82_cropped.jpg} \\

{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_340_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_368_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_152_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_82_norm.jpg} \\

% Tunnel
{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_144944_324_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_495_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164537_75_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_0_cropped.jpg} \\

{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_144944_324_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_495_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164537_75_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_0_norm.jpg} \\

%560 is left out
% Sharp
{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_422_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_48_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164345_97_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_188_cropped.jpg} \\

{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_422_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_48_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164345_97_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/qualitative/20190614_164848_188_norm.jpg} \\
\end{tabular}


==> img/fisheye_fig/syndistnet_fisheye.tex <==
\newcommand{\turnheightnew}{0.25\columnwidth}
\centering

\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

{\rotatebox{90}{\hspace{4mm}Raw Input}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/infinite_depth/20190614_143708_506_crop.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/infinite_depth/20190614_163808_146_crop.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/semantic_guidance_dc_mask/20190614_144708_1144_crop.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/semantic_guidance_dc_mask/0000000286_crop.jpg}\\

{\rotatebox{90}{\hspace{4mm}Baseline}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/infinite_depth/20190614_143708_506_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/infinite_depth/20190614_163808_146_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/semantic_guidance_dc_mask/20190614_144708_1144_orig_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/semantic_guidance_dc_mask/0000000286_orig_norm.jpg}\\

{\rotatebox{90}{\hspace{3mm}SynDistNet}} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/infinite_depth/20190614_143708_506_orig_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/infinite_depth/20190614_163808_146_orig_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/semantic_guidance_dc_mask/20190614_144708_1144_norm.jpg} &
\includegraphics[height=\turnheightnew]{img/fisheye_fig/semantic_guidance_dc_mask/0000000286_norm.jpg} \\

\end{tabular}

==> img/kitti_fig/kitti.tex <==
\newcommand{\turnheightnew}{0.25\columnwidth}
\centering

\begin{tabular}{c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

\Large Raw Input &
\Large Zhou \cite{zhou2017unsupervised} &
\Large Godard \cite{Godard2019} &
\Large SynDistNet\\

\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/rgb_image_0546.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_zhou_image_0546.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_godard_image_0546.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_pred_image_0546.png}\\

\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/rgb_image_0592.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_zhou_image_0592.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_godard_image_0592.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_pred_image_0592.png}\\

\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/rgb_image_0388.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_zhou_image_0388.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_godard_image_0388.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_pred_image_0388.png}\\

\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/rgb_image_0099.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_zhou_image_0099.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_godard_image_0099.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_pred_image_0099.png}\\

\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/rgb_image_0645.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_zhou_image_0645.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_godard_image_0645.png}\; &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs/depth_pred_image_0645.png}\\

\end{tabular}

==> img/kitti_fig/kitti_fig.tex <==
\newcommand{\turnheightnew}{0.23\columnwidth}
\centering

\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

{\rotatebox{90}{\hspace{5mm}\normalsize
{Input}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_color.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_color.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_color.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_color.jpg}\\

{\rotatebox{90}{\hspace{0mm}\small
{Monodepth~\cite{Godard2017}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_monodepth_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_monodepth_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_monodepth_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_monodepth_disp.jpg} \\

{\rotatebox{90}{\hspace{0mm}\small
{Zhou \etal~\cite{zhou2017unsupervised}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_zhou_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_zhou_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_zhou_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_zhou_disp.jpg} \\

{\rotatebox{90}{\hspace{2mm}\small
{DDVO~\cite{Wang2018e}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_posenet_ddvo_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_posenet_ddvo_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_posenet_ddvo_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_posenet_ddvo_disp.jpg} \\

{\rotatebox{90}{\hspace{2mm}\small
{GeoNet~\cite{Yin2018}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_geonet_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_geonet_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_geonet_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_geonet_disp.jpg} \\

{\rotatebox{90}{\hspace{0mm}\small
{Zhan \etal~\cite{zhan2018unsupervised}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_zhan_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_zhan_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_zhan_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_zhan_disp.jpg} \\

{\rotatebox{90}{\hspace{0mm}\small
Ranjan et al.~\cite{Ranjan2019}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_gan_adv_col_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_gan_adv_col_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_gan_adv_col_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_gan_adv_col_disp.jpg} \\


{\rotatebox{90}{\hspace{0mm} \small
3Net-R50~\cite{Luo2019a}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_3net_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_3net_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_3net_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_3net_disp.jpg} \\ 

{\rotatebox{90}{\hspace{0mm} \small
EPC++ (MS) \newline \cite{Luo2019a}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_epcpp_ms_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_epcpp_ms_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_epcpp_ms_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_epcpp_ms_disp.jpg} \\ 

{\rotatebox{90}{\hspace{0mm}\small
Monodepth2 M~\cite{Godard2019}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_monodepth2_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_monodepth2_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_monodepth2_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_monodepth2_disp.jpg} \\

{\rotatebox{90}{\hspace{3mm}\small
\textbf{SVDistNet}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0084_sync_283_ours_depth.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0036_sync_64_ours_depth.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0046_sync_110_ours_depth.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/qualitative/2011_09_26_drive_0106_sync_43_ours_depth.jpg} \\

\end{tabular}


==> img/kitti_fig/kitti_sem.tex <==
\newcommand{\turnheightnew}{0.25\columnwidth}
\centering
\large
\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

{\rotatebox{90}{\hspace{2mm}Raw Input}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/rgb_baseline_image011.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/rgb_baseline_image043.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/rgb_baseline_image136.png} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/rgb_baseline_image166.png}\\

{\rotatebox{90}{\hspace{2mm}SVDistNet}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/depth_predicted011.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/depth_predicted043.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/depth_predicted136.png} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/depth_predicted166.png}\\

{\rotatebox{90}{\hspace{1mm}SVDistNet}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/sem_predicted_image011.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/sem_predicted_image043.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/sem_predicted_image136.png} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/sem_predicted_image166.png} \\

{\rotatebox{90}{\hspace{2mm}Raw Input}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/rgb_baseline_image000.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/rgb_baseline_image070.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/rgb_baseline_image090.png} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/rgb_baseline_image140.png}\\

{\rotatebox{90}{\hspace{2mm}SVDistNet}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/depth_predicted000.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/depth_predicted070.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/depth_predicted090.png} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/depth_predicted140.png}\\

{\rotatebox{90}{\hspace{1mm}SVDistNet}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/sem_predicted_image000.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/sem_predicted_image070.png} &
%\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/sem_predicted_image090.png} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/imgs_sem/sem_predicted_image140.png} \\

\end{tabular}

==> img/post_processing/post_processing_v1.tex <==
\centering
\begin{tabular}{@{\hskip 0.5mm}c@{}}

\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-11h50m49s962.png} \\
\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-11h51m31s816.png} \\
\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-11h52m13s070.png} \\

\end{tabular}


==> img/post_processing/post_processing_v2.tex <==
\centering
\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-11h53m42s103_crop.jpg} \\
\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-11h52m41s488_crop.jpg} \\
\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-11h53m58s395_crop.jpg} \\
\end{tabular}


==> img/post_processing/post_processing_v3.tex <==
\centering
\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-12h03m45s520.png} \\
\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-12h17m24s965.png} \\
\end{tabular}


==> img/post_processing/post_processing_v4.tex <==
\centering
\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-12h03m13s878.png} &
\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-12h03m09s132.png} &
\includegraphics[height=\textwidth]{img/post_processing/vlcsnap-2020-09-07-12h03m17s159.png} \\

\end{tabular}


==> results/ate_error.tex <==
\begin{table}[!t]
\centering
\begin{adjustbox}{width=\columnwidth}
\captionsetup{belowskip=-16pt, skip=4pt, font= small, singlelinecheck=false}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{l}{\textbf{Method}} 
& \textit{\begin{tabular}[c]{@{}c@{}}No. of\\ Frames\end{tabular}} 
& \textit{GT} 
& \cellcolor[HTML]{7d9ebf}\textit{Sequence 09} 
& \cellcolor[HTML]{e8715b}\textit{Sequence 10} \\ 
\midrule
    ORB-SLAM~\cite{mur2015orb}                   & 5 & \ch & 0.014 $\pm$ 0.008 & 0.012 $\pm$ 0.011 \\
    DF-Net~\cite{zou2018df}                      & 5 & \ch & 0.017 $\pm$ 0.007 & 0.015 $\pm$ 0.009 \\
    SfMLearner~\cite{zhou2017unsupervised}       & 5 & \ch & 0.016 $\pm$ 0.009 & 0.013 $\pm$ 0.009 \\
    Klodt et al.~\cite{klodt2018supervising}     & 5 & \ch & 0.014 $\pm$ 0.007 & 0.013 $\pm$ 0.009 \\
    GeoNet~\cite{Yin2018}                        & 5 & \ch & 0.012 $\pm$ 0.007 & 0.012 $\pm$ 0.009 \\
    Struct2Depth~\cite{Casser2019}               & 5 & \ch & 0.011 $\pm$ 0.006 & 0.011 $\pm$ 0.010 \\
    Ranjan~\cite{Ranjan2019}                     & 5 & \ch & 0.011 $\pm$ 0.006 & 0.011 $\pm$ 0.010 \\ 
    PackNet-SfM~\cite{Guizilini2020a}            & 5 & \ch & 0.010 $\pm$ 0.005 & 0.009 $\pm$ 0.008 \\
    PackNet-SfM~\cite{Guizilini2020a}            & 5 & \xm & 0.014 $\pm$ 0.007 & 0.012 $\pm$ 0.008 \\
    SVDistNet                                      & 5 & \ch & \textbf{0.009} $\pm$ \textbf{0.004} & 0.008 $\pm$ \textbf{0.005} \\
    SVDistNet                                      & 5 & \xm & 0.010 $\pm$ 0.005 & 0.010 $\pm$ 0.008 \\
    \midrule
    DDVO~\cite{Wang2018e}                        & 3 & \ch & 0.045 $\pm$ 0.108 & 0.033 $\pm$ 0.074 \\
    Vid2Depth~\cite{mahjourian2018unsupervised}  & 3 & \ch & 0.013 $\pm$ 0.010 & 0.012 $\pm$ 0.011 \\
    EPC++~\cite{Luo2019a}                        & 3 & \ch & 0.013 $\pm$ 0.007 & 0.012 $\pm$ 0.008 \\
    SVDistNet                                      & 3 & \ch & \textbf{0.011} $\pm$ \textbf{0.006} & \textbf{0.010} $\pm$ \textbf{0.007} \\
    SVDistNet                                      & 3 & \xm & 0.012 $\pm$ 0.007 & 0.011 $\pm$ 0.008 \\
    \midrule
    Monodepth2~\cite{Godard2019}                   & 2 & \ch & 0.017 $\pm$ 0.008 & 0.015 $\pm$ 0.010 \\
    SVDistNet                                      & 2 & \ch & \textbf{0.015} $\pm$ \textbf{0.007} & \textbf{0.013} $\pm$ \textbf{0.007} \\
    SVDistNet                                      & 2 & \xm & 0.016 $\pm$ 0.008 & 0.014 $\pm$ 0.009 \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
\caption{\textbf{Evaluation of the pose estimation} on the KITTI Odometry Benchmark~\cite{geiger2013vision}.}
\label{table:supplementary-pose-ate}
\vspace{-2em}
\end{table}


==> results/inference_onnx.tex <==
\begin{table}[t]
\captionsetup{belowskip=-6pt, skip=4pt, font= small, singlelinecheck=false}
\centering
  \small
    \setlength{\tabcolsep}{0.2em}
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Method} & \textit{Dataset} & 
    \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} \textit{Network} \\ \textit{Resolution} \end{tabular}} &
    \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} \textit{Encoder} \\ \textit{head} \end{tabular}} &
    \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} \textit{Inference} \\ \textit{(fps)} \end{tabular}} \\
    \toprule
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} FisheyeDistanceNet~\cite{kumar2020fisheyedistancenet}\end{tabular}}
      & K  & 640 x 192  & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} ResNet-18\end{tabular}} & 84 \\
      & K  & 1024 x 320 &                                                                     & 34 \\
      & WS & 512 x 256  &                                                                     & 89 \\
    \midrule
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} UnrectDepthNet~\cite{kumar2020unrectdepthnet}\end{tabular}}
      & K  & 640 x 192  & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} ResNet-50\end{tabular}} & 39 \\
      & K  & 1024 x 320 &                                                                     & 16 \\
      & WS & 512 x 256  &                                                                     & 42 \\
      & WS & 1024 x 512 &                                                                     & 11 \\
    \midrule  
    \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} SynDistNet~\cite{kumar2020syndistnet}\end{tabular}}
      & K  & 640 x 192  & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} ResNet-18\end{tabular}} & 82 \\
      & K  & 1024 x 320 &                                                                     & 33 \\
      & WS & 512 x 256  &                                                                     & 91 \\
      & WS & 1024 x 512 &                                                                     & 23 \\
      & WS & 512 x 256  & ResNet50                                                            & 42 \\
      \midrule
    \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} SVDistNet \end{tabular}}
      & K  & 640 x 192  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} SAN-10\end{tabular}} & 80 \\
      & K  & 1024 x 320 &                                                                  & 30 \\
      & WS & 512 x 256  &                                                                  & 87 \\
      & WS & 512 x 256  & SAN-19                                                           & 45 \\
    \bottomrule
\end{tabular}
\caption{\textbf{Ablation study on inference time (frames per second)} using ONNX 16-bit float precision models on NVIDIA's Jetson AGX device of FisheyeDistanceNet~\cite{kumar2020fisheyedistancenet}, UnrectDepthNet~\cite{kumar2020unrectdepthnet}, SynDistNet \cite{kumar2020syndistnet} and SVDistNet on the KITTI (K) and WoodScape (WS) datasets.}
\label{table:inference-ablation}
\end{table} 

==> results/kittti_big_quantitative.tex <==
\begin{table*}[!ht]
\captionsetup{belowskip=-12pt, font= small, singlelinecheck=false}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|llccccccc}
\toprule
& \multirow{2}{*}{\textbf{Method}}
& Train
& \cellcolor[HTML]{7d9ebf}Abs Rel & \cellcolor[HTML]{7d9ebf}Sq Rel & \cellcolor[HTML]{7d9ebf}RMSE & \cellcolor[HTML]{7d9ebf}RMSE$_{log}$ & \cellcolor[HTML]{e8715b}$\delta<1.25$ & \cellcolor[HTML]{e8715b}$\delta<1.25^2$ & \cellcolor[HTML]{e8715b}$\delta<1.25^3$ \\
\cmidrule(lr){4-7} \cmidrule(lr){8-10}
& & & \multicolumn{4}{c}{\cellcolor[HTML]{7d9ebf}lower is better} & \multicolumn{3}{c}{\cellcolor[HTML]{e8715b}higher is better} \\
\toprule
\parbox[t]{2mm}{\multirow{33}{*}{\rotatebox[origin=c]{90}{Original~\cite{Eigen_14}}}}
& SfMLearner~\cite{zhou2017unsupervised}      & M & 0.208 & 1.768 & 6.958 & 0.283 & 0.678 & 0.885 & 0.957 \\
& DNC~\cite{yang2017unsupervised}             & M & 0.182 & 1.481 & 6.501 & 0.267 & 0.725 & 0.906 & 0.963 \\
& Vid2Depth~\cite{mahjourian2018unsupervised} & M & 0.163 & 1.240 & 6.220 & 0.250 & 0.762 & 0.916 & 0.968 \\
& LEGO~\cite{yang2018lego}                    & M & 0.162 & 1.352 & 6.276 & 0.252 & 0.783 & 0.921 & 0.969 \\
& Kumar~\cite{Kumar2018a}                & M & 0.211 & 1.979 & 6.154 & 0.263 & 0.731 & 0.897 & 0.959 \\
& Wang \etal~\cite{wang2019unsupervised}      & M & 0.158 & 1.277 & 5.858 & 0.233 & 0.785 & 0.929 & 0.973 \\
& GeoNet~\cite{Yin2018}                       & M & 0.155 & 1.296 & 5.857 & 0.233 & 0.793 & 0.931 & 0.973 \\
& Cycle-SfM~\cite{sun2019cycle}               & M & 0.162 & 1.349 & 5.847 & 0.239 & 0.784 & 0.925 & 0.969 \\
& Li \etal~\cite{li2019sequential}            & M & 0.150 & 1.127 & 5.564 & 0.229 & 0.823 & 0.936 & 0.974 \\
& DDVO~\cite{Wang2018e}                & M & 0.151 & 1.257 & 5.583 & 0.228 & 0.810 & 0.936 & 0.974 \\
& DF-Net~\cite{zou2018df}                     & M & 0.150 & 1.124 & 5.507 & 0.223 & 0.806 & 0.933 & 0.973 \\
& GANVO~\cite{almalioglu2019ganvo}            & M & 0.150 & 1.141 & 5.448 & 0.216 & 0.808 & 0.939 & 0.975 \\
& Bian~\cite{bian2019unsupervised}            & M & 0.137 & 1.089 & 5.439 & 0.217 & 0.830 & 0.942 & 0.975 \\
& EPC++~\cite{Yang2018c}                      & M & 0.141 & 1.029 & 5.350 & 0.216 & 0.816 & 0.941 & 0.976 \\
& CC~\cite{Ranjan2019}             & M & 0.140 & 1.070 & 5.326 & 0.217 & 0.826 & 0.941 & 0.975 \\
& Struct2Depth~\cite{Casser2019}              & M & 0.141 & 1.036 & 5.291 & 0.215 & 0.816 & 0.945 & 0.979 \\
& LearnK~\cite{Gordon2019}                    & M & 0.128 & 0.959 & 5.230 & 0.212 & 0.845 & 0.947 & 0.976 \\
& SIGNet~\cite{Meng2019a}                & M & 0.133 & 0.905 & 5.181 & 0.208 & 0.825 & 0.947 & 0.981 \\
& DualNet~\cite{Zhou2019}                     & M & 0.121 & 0.837 & 4.945 & 0.197 & 0.853 & 0.955 & 0.982 \\
& OmegaNet~\cite{tosi2020distilled}           & M & 0.126 & 0.835 & 4.937 & 0.199 & 0.844 & 0.953 & 0.982 \\
& SuperDepth~\cite{pillai2019superdepth}      & M & 0.116 & 1.055 & -     & 0.209 & 0.853 & 0.948 & 0.977 \\
& Monodepth2~\cite{Godard2019}                & M & 0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981 \\
& PackNet-SfM~\cite{Guizilini2020a}           & M & 0.111 & 0.829 & 4.788 & 0.199 & 0.864 & 0.954 & 0.980 \\
& FisheyeDistanceNet~\cite{kumar2020fisheyedistancenet} & M & 0.117 & 0.867 & 4.739 & 0.190 & 0.869 & 0.960 & 0.982 \\
& SGDepth~\cite{Klingner2020}                 & M & 0.113 & 0.880 & 4.695 & 0.192 & 0.884 & 0.961 & 0.981 \\
& Patil \etal~\cite{patil2020don}             & M & 0.111 & 0.821 & 4.650 & 0.187 & 0.883 & 0.961 & 0.982 \\
& UnRectDepthNet~\cite{kumar2020unrectdepthnet} & M & 0.107 & 0.721 & 4.564 & 0.178 & 0.894 & 0.971 & 0.986 \\
& SynDistNet~\cite{kumar2020syndistnet}       & M & 0.109 & 0.718 & 4.516 & 0.180 & 0.896 & 0.973 & 0.986 \\
& Shu \etal~\cite{shu2020featdepth}           & M & 0.104 & 0.729 & 4.481 & 0.179 & 0.893 & 0.965 & 0.984 \\
& \textbf{SVDistNet}                          & M & \textbf{0.102} & \textbf{0.706} & \textbf{4.459} & \textbf{0.172} & \textbf{0.908} & \textbf{0.974} & \textbf{0.986} \\
\cmidrule{2-10}
& Struct2Depth~\cite{Casser2019}             & M${^*}$ & 0.109 & 0.825 & 4.750 & 0.187 &0.874 & 0.958 & 0.983 \\
& GLNet~\cite{Chen2019b}                  & M$^{*}$ & 0.099 & 0.796 & 4.743 & 0.186 &0.884 & 0.955 & 0.979 \\
& Shu \etal~\cite{shu2020featdepth}          & M$^{*}$ & 0.088 & 0.712 & 4.137 & \textbf{0.169} & 0.915 & 0.965 & 0.982 \\
& \textbf{SVDistNet}                         & M${^*}$ & \textbf{0.086} & \textbf{0.701} & \textbf{4.118} & 0.170 & \textbf{0.919} & \textbf{0.976} & \textbf{0.985} \\
\midrule
\parbox[t]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{Improved~\cite{uhrig2017sparsity}}}}
& SfMLearner~\cite{zhou2017unsupervised}    & M & 0.176 & 1.532 & 6.129 & 0.244 & 0.758 & 0.921 & 0.971 \\
& Vid2Depth~\cite{mahjourian2018unsupervised} & M & 0.134 & 0.983 & 5.501 & 0.203 & 0.827 & 0.944 & 0.981 \\
& GeoNet~\cite{Yin2018}                     & M & 0.132 & 0.994 & 5.240 & 0.193 & 0.883 & 0.953 & 0.985 \\
& DDVO~\cite{Wang2018e}              & M & 0.126 & 0.866 & 4.932 & 0.185 & 0.851 & 0.958 & 0.986 \\
& EPC++~\cite{Yang2018c}                    & M & 0.120 & 0.789 & 4.755 & 0.177 & 0.856 & 0.961 & 0.987 \\
& Monodepth2~\cite{Godard2019}              & M & 0.090 & 0.545 & 3.942 & 0.137 & 0.914 & 0.983 & 0.995 \\
& PackNet-SfM~\cite{Guizilini2020a}         & M & 0.078 & 0.420 & 3.485 & 0.121 & 0.931 & 0.986 & 0.996 \\
& UnRectDepthNet~\cite{kumar2020unrectdepthnet} & M & 0.081 & 0.414 & 3.412 & 0.117 & 0.926 & 0.987 & 0.996 \\
& SynDistNet~\cite{kumar2020syndistnet}     & M & 0.076 & 0.412 & 3.406 & 0.115 & 0.931 & 0.988 & 0.996 \\
& \textbf{SVDistNet}                        & M & \textbf{0.071} & \textbf{0.405} & \textbf{3.345} & \textbf{0.106} & \textbf{0.934} & \textbf{0.988} & \textbf{0.996} \\
& \textbf{SVDistNet}                        & M${^*}$ & \textbf{0.059} & \textbf{0.392} & \textbf{3.206} & \textbf{0.097} & \textbf{0.935} & \textbf{0.989} & \textbf{0.995} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Evaluation of the KITTI Eigen split} compared to most of the previous self-supervised monocular depth estimation methods. Following best practices, we cap depths at 80\,m. We also evaluate using the \textit{Original} depth maps generated from raw point clouds as proposed by \cite{Eigen_14} as well as \textit{Improved} annotated depth maps as introduced by \cite{uhrig2017sparsity}. M indicates that sequences are trained on using the monocular approach. M${^*}$ indicates the online refinement technique~\cite{Casser2019}, where the model is trained during the inference. Note that while most approaches use median scaling concerning the ground truth at test-time for a scale-consistent prediction, we do not need to use this scaling method.}
\label{tab:kitti-monocular-results}
\end{table*}

==> results/metrics_formulas.tex <==
\begin{table*}[htpb]
\centering
\captionsetup{belowskip=-12pt, font= small, singlelinecheck=false}
\scalebox{1.25}{
\begin{tabular}{ll}
\toprule
$\textbf{Abs Rel}: \frac{1}{|N|}\sum_{i\in N}\frac{\mid d_{i}-d_{i}^{*}\mid}{d_{i}^{*}}$
&$\textbf{RMSE}:\sqrt{\frac{1}{|N|}\sum_{i\in N}\parallel d_{i}-d_{i}^{*} \parallel^{2}}$\\
$\textbf{Sq Rel}:\frac{1}{|N|}\sum_{i\in N}\frac{\parallel d_{i}-d_{i}^{*}\parallel^{2}}{d_{i}^{*}}$
&$\textbf{RMSE log}: \sqrt{\frac{1}{|N|}\sum_{i\in N}\parallel \log (d_{i})- \log (d_{i}^{*}) \parallel^{2}}$ \\
\multicolumn{2}{l}{\textbf{Accuracies} $\mathbf{\delta}_\mathbf{t}:
\frac{1}{|N|}|\{d \in N| \: \max(\frac{d_{i}}{d_{i}^{*}}, \frac{d_{i}^{*}}{d_{i}}) \: < 1.25^t\}|\times 100\%$} \\
\bottomrule
\end{tabular}
}
\caption{Performance indicators for depth evaluation. where $d_{i}$ and  $d_{i}^{*}$ denotes the predicted and ground truth depth value of pixel $i$ respectively. $N$ denotes the set of a total number of pixels with real-depth/distance values in an image, $|.|$ returns the number of the input set elements.}
\end{table*}

==> results/online_refinement.tex <==
\begin{table}[t!]
\captionsetup{belowskip=-10pt, skip=4pt, font= small, singlelinecheck=false}
\centering
\small
\begin{adjustbox}{width=\columnwidth}
\setlength{\tabcolsep}{0.1em}
  \begin{tabular}{lccccccc}
	\toprule
    \multirow{2}{*}{\textbf{Method}} &
    \cellcolor[HTML]{7d9ebf}Abs Rel & \cellcolor[HTML]{7d9ebf}Sq Rel & \cellcolor[HTML]{7d9ebf}RMSE & \cellcolor[HTML]{7d9ebf}RMSE$_{log}$ & \cellcolor[HTML]{e8715b}$\delta<1.25$ & \cellcolor[HTML]{e8715b}$\delta<1.25^2$ & \cellcolor[HTML]{e8715b}$\delta<1.25^3$ \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-8}
    &  \multicolumn{4}{c}{\cellcolor[HTML]{7d9ebf}lower is better} & \multicolumn{3}{c}{\cellcolor[HTML]{e8715b}higher is better} \\
    \toprule
     SAN10-patch & 0.044 & 0.302 & 1.274 & 0.097 & 0.906 & 0.987 & 0.995 \\
     SAN10-pair  & 0.069 & 0.353 & 1.543 & 0.111 & 0.901 & 0.985 & 0.993 \\
     SAN19-patch & 0.034 & 0.264 & 1.218 & 0.073 & 0.914 & 0.992 & 0.996 \\
     SAN19-pair  & 0.065 & 0.322 & 1.545 & 0.092 & 0.896 & 0.988 & 0.995 \\
    \bottomrule
  \end{tabular}
\end{adjustbox}
\caption{\textbf{Online refinement} of the network's distance estimates incorporating~\cite{Casser2019}, where the model is trained during the inference as well on WoodScape dataset.~\cite{yogamani2019woodscape}.}
\label{table:online-refine}
\end{table}
\vspace{-1em}

==> results/optimizer.tex <==
\begin{table}[t]
\captionsetup{belowskip=-4pt, skip=4pt, font= small, singlelinecheck=false}
\centering
\small
\begin{adjustbox}{width=\columnwidth}
\setlength{\tabcolsep}{0.2em}
  \begin{tabular}{lccccccc}
	\toprule
    \multirow{2}{*}{\textbf{Optimizer}} &
    \cellcolor[HTML]{5880ab}Abs Rel & \cellcolor[HTML]{5880ab}Sq Rel & \cellcolor[HTML]{5880ab}RMSE & \cellcolor[HTML]{5880ab}RMSE$_{log}$ & \cellcolor[HTML]{e8715b}$\delta<1.25$ & \cellcolor[HTML]{e8715b}$\delta<1.25^2$ & \cellcolor[HTML]{e8715b}$\delta<1.25^3$ \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-8}
    &  \multicolumn{4}{c}{\cellcolor[HTML]{5880ab}lower is better} & \multicolumn{3}{c}{\cellcolor[HTML]{e8715b}higher is better} \\
    \toprule
     Adam    & 0.069 & 0.338 & 1.551 & 0.118 & 0.887 & 0.980 & 0.991 \\
     Ranger  & 0.057 & 0.315 & 1.532 & 0.108 & 0.896 & 0.987 & 0.996 \\
    \bottomrule
  \end{tabular}
\end{adjustbox}
\caption{\textbf{Impact of the optimizer} on WoodScape dataset.~\cite{yogamani2019woodscape}.}
\label{table:optimizer}
\end{table}

==> results/robust_loss_ablation.tex <==
\begin{table}[!t]
\captionsetup{belowskip=-6pt, skip=4pt, font= small, singlelinecheck=false}
\centering
  \small
  \begin{adjustbox}{width=\columnwidth}
    \setlength{\tabcolsep}{0.1em}
	  \begin{tabular}{llccccccc}
	    \toprule
        \multirow{2}{*}{\textbf{Method}}  & \multirow{2}{*}{$\alpha$} & \cellcolor[HTML]{7d9ebf}Abs Rel & \cellcolor[HTML]{7d9ebf}Sq Rel & \cellcolor[HTML]{7d9ebf}RMSE & \cellcolor[HTML]{7d9ebf}RMSE$_{log}$ & \cellcolor[HTML]{e8715b}$\delta<1.25$ & \cellcolor[HTML]{e8715b}$\delta<1.25^2$ & \cellcolor[HTML]{e8715b}$\delta<1.25^3$ \\
        \cmidrule(lr){3-6} \cmidrule(lr){7-9}
        & & \multicolumn{4}{c}{\cellcolor[HTML]{7d9ebf}lower is better} & \multicolumn{3}{c}{\cellcolor[HTML]{e8715b}higher is better} \\
	    \toprule
	    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} SynDistNet \end{tabular}}   
	    & 2    & 0.154 & 0.631 & 2.532 & 0.198 & 0.832 & 0.965 & 0.981 \\
        & 0, 2 & 0.142 & 0.537 & 2.316 & 0.179 & 0.878 & 0.971 & 0.985 \\
        \midrule
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} SVDistNet \end{tabular}}       
        & 2    & 0.145 & 0.564 & 2.279 & 0.186 & 0.863 & 0.966 & 0.982 \\
        & 0, 2 & 0.128 & 0.469 & 2.153 & 0.164 & 0.875 & 0.974 & 0.986 \\
	   \bottomrule
    \end{tabular}
  \end{adjustbox}
\caption{\textbf{Impact of using the robust loss function} compared to the baseline from \cite{kumar2020syndistnet} on the Fisheye WoodScape dataset~\cite{yogamani2019woodscape}.}
%We witness significant performance gains when replacing the \lone loss with various variants of the robust loss function.}
\label{table:robust-ablation}
\end{table}

